Neural Network Learner for Minesweeper

Minesweeper is an interesting single player game based on logic, memory and guessing. Solving Minesweeper has been shown to be an NP-hard task. Deterministic solvers are the best known approach for solving Minesweeper. This project proposes a neural network based learner for solving Minesweeper. To choose the best learner, different architectures and configurations of neural networks were trained on hundreds of thousands of games. Surprisingly, the proposed neural network based learner has shown to be a very good approximation function for solving Minesweeper. The neural network learner competes well with the CSP solvers, especially in Beginner and Intermediate modes of the game. It was also observed that despite having high success rates, the best neural learner was considerably slower than the best deterministic solver. This report also discusses the overheads and limitations faced while creating highly successful neural networks for Minesweeper.

==> chapters/discussion.tex <==
\chapter{Discussion and Analysis}
\label{ch:evaluation}

Depending on the type of project you are doing, this chapter can be merged with ``Results'' Chapter as `` Results and Discussion'' as suggested by your supervisor. 

In the case of software development and the standalone applications, describe the significance of the obtained results/performance of the system. 



\section{A section}% please use an appropriate section title
Discussion and analysis chapter evaluates and analyses the results. It interprets the obtained results. 



\section{Significance of the findings}
In this chapter, you should also try to discuss the significance of the results and key findings, in order to enhance the reader's understanding of the investigated problem

\section{Limitations} % please discuss limitation of the project 
Discuss the key limitations and potential implications or improvements of the findings.
\section{Summary}
Write a summary of this chapter.

==> chapters/reflection.tex <==
\chapter{Reflection}
\label{ch:reflection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please remove/replace text below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Write a short paragraph on the substantial learning experience. This can include your decision-making approach in problem-solving.

\textbf{Some hints:} You obviously learned how to use different programming languages, write reports in \LaTeX and use other technical tools. In this section, we are more interested in what you thought about the experience. Take some time to think and reflect on your individual project as an experience, rather than just a list of technical skills and knowledge. You may describe things you have learned from the research approach and strategy, the process of identifying and solving a problem, the process research inquiry, and the understanding of the impact of the project on your learning experience and future work.

Also think in terms of:
\begin{itemize}
    \item what knowledge and skills you have developed
    \item what challenges you faced, but was not able to overcome
    \item what you could do this project differently if the same or similar problem would come
    \item rationalize the divisions from your initial planed aims and objectives.
\end{itemize}


A good reflective summary could be approximately 300--500 words long, but this is just a recommendation.

~\\[2em]
\noindent
{\huge \textbf{Note:}} The next chapter is ``\textbf{References},'' which will be automatically generated if you are using BibTeX referencing method. This template uses BibTeX referencing.  Also, note that there is difference between ``References'' and ``Bibliography.'' The list of ``References'' strictly only contain the list of articles, paper, and content you have cited (i.e., refereed) in the report. Whereas Bibliography is a list that contains the list of articles, paper, and content you have cited in the report plus the list of articles, paper, and content you have read in order to gain knowledge from. We recommend to use only the list of ``References.'' 


==> chapters/results.tex <==
\chapter{Results}
\label{ch:results}
The results chapter tells a reader about your findings based on the methodology you have used to solve the investigated problem. For example: 
\begin{itemize}
    \item If your project aims to develop a software/web application, the results may be the developed software/system/performance of the system, etc., obtained using a relevant methodological approach in software engineering. 
    
    \item If your project aims to implement an algorithm for its analysis, the results may be the performance of the algorithm obtained using a relevant experiment design. 
    
    \item If your project aims to solve some problems/research questions over a collected dataset, the results may be the findings obtained using the applied tools/algorithms/etc. 
\end{itemize}
Arrange your results and findings in a logical sequence. 



\section{A section}

...

\clearpage
\section{Example of a Table in \LaTeX}
Table~\ref{tab:_ex_tab} is an example of a table created using the package \LaTeX  ``booktabs.'' do check the link: \href{https://en.wikibooks.org/wiki/LaTeX/Tables}{wikibooks.org/wiki/LaTeX/Tables} for more details. A table should be clean and readable. Unnecessary horizontal lines and vertical lines in tables make them unreadable and messy. The example in Table~\ref{tab:_ex_tab} uses a minimum number of liens (only necessary ones). Make sure that the top rule and bottom rule (top and bottom horizontal lines) of a table are present. 

\begin{table}[h!]
    \centering
    \caption{Example of a table in \LaTeX}
    \label{tab:_ex_tab}
    \begin{tabular}{llr}     
        \toprule
        \multicolumn{2}{c}{Bike} \\
        \cmidrule(r){1-2}
        Type    &  Color & Price (\pounds) \\
        \midrule
        Electric    & black   & 700   \\
        Hybrid      & blue    & 500   \\
        Road        & blue    & 300   \\
        Mountain    & red     & 300   \\
        Folding     & black   & 500   \\
        \bottomrule
    \end{tabular}
\end{table}

\section{Example of captions style}

\begin{itemize}
    \item The \textbf{caption of a Figure (artwork) goes below} the artwork (Figure/Graphics/illustration). See example artwork in Figure~\ref{fig:chart_a}. 
    \item  The \textbf{caption of a Table goes above} the table. See the example in Table~\ref{tab:_ex_tab}.
    \item  The \textbf{caption of an Algorithm goes above} the algorithm. See the example in Algorithm~\ref{algo:algo_example}.
    \item The \textbf{caption of a Listing goes below} the Listing  (Code snippet). See example listing in Listing~\ref{list:python_code_ex}. 
\end{itemize} 





\section{Summary}
Write a summary of this chapter.





==> chapters/rule_induction.tex <==
\chapter{Rule induction}

==> glossaries.tex <==
\chapter*{List of Abbreviations}
\chaptermark{List of Abbreviations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Enter your list of Abbreviation and Symbols in this file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abbrv}
    
    \item[SMPCS]			School of Mathematical, Physical and Computational Sciences
    
\end{abbrv}

